Forecasting dynamic return distributions based on ordered binary choice

We present a simple approach to forecasting conditional probability distributions of asset returns. We work with a parsimonious specification of ordered binary choice regression that imposes a connection on sign predictability across different quantiles. The model forecasts the future conditional probability distributions of returns quite precisely when using a past indicator and past volatility proxy as predictors. Direct benefits of the model are revealed in an empirical application to the 29 most liquid U.S. stocks. The forecast probability distribution is translated to significant economic gains in a simple trading strategy. Our approach can also be useful in many other applications where conditional distribution forecasts are desired.

==> Ordered_RR_figures_core_Fin.tex <==




\section{Figures: Parameter Estimates}


\begin{figure}[!h]
\centering
\includegraphics[width=4.8in]{parameter_plot_2}
\caption{Parameter estimates: ordered logit parameters estimated for all 29 stocks shown by box-and-whisker plots.}
\label{fig:pars1}
\end{figure}

\begin{figure}[!h]
\centering
\includegraphics[width=\textwidth]{parameter_plot_1_Fin}
\caption{Parameter estimates: coefficient functions implied by parameters estimated for all 29 stocks. Minimum and maximum values shown as light grey area, 50\% of distribution as grey area, and median as black line.}
\label{fig:pars2}
\end{figure}

\clearpage
\newpage
\section{Figures: Conditional CDF}
\vspace{2cm}

\begin{figure}[!h]
\centering
\includegraphics[width=0.75\textwidth]{CDF_plot_Fin}
\par\bigskip\bigskip
\caption{Fragment of interpolated estimated conditional CDF of returns for one of stocks.}
\label{fig:CDFplot}
\end{figure}

\clearpage
\newpage
\section{Figures: Statistical Evaluation}

\begin{figure}[!h]
\centering
\includegraphics[width=0.45 \textwidth]{GR_plot1}
\caption{p-values from Gonzalez-Rivera and Sun (2015) tests for ordered logit model shown by box-and-whisker plots for all 29 stocks. Four test specifications are shown with $\alpha = (0.25,0.5,0.75)'$ (a) contour-aggregated, (b) lag-aggregated, with $\alpha = (0.05,0.1,...,0.9,0.95)'$ (c) contour-aggregated, (d) lag-aggregated.}
\label{fig:testplot}
\end{figure}

\begin{figure}[!h]
\centering
\includegraphics[width=0.9\textwidth]{scores_plot}
\caption{Brier scores and CRPS for ordered logit (1), separate logits (2), GARCH (3), and FHS (4) shown by box-and-whisker plots for all 29 stocks. Larger values of the scores are preferred to their smaller values.}
\label{fig:scoresplot}
\end{figure}


\clearpage
\section{Figures: Economic Evaluation}

\begin{figure}[!h]
\centering
\includegraphics[width=\textwidth]{trading_plot}
\caption{Performance of ordered logit (1), separate logits (2), market benchmark (3), GARCH (4), and FHS (5) models. Return, volatility and Sharpe ratio for all 29 stocks are shown by box-and-whisker plots.}
\label{fig:tradingplot}
\end{figure}

\begin{sidewaysfigure}[!ht]
\centering
\includegraphics[width=3in]{Probability_Strategy_figure_13}
\includegraphics[width=3in]{Probability_Strategy_figure_24}
\includegraphics[width=3in]{Probability_Strategy_figure_30}
\caption{Performance: cumulative return and drawdown for three typical stocks. Trading strategy based on probability predictions from ordered logit model in purple ({\color{purple}{ $\boldsymbol{ -}$ }}), separate logits in bordeaux ({\color{bordeaux}{ $\boldsymbol{-}$ }}), GARCH in red ({\color{red}{ $\boldsymbol{-}$ }}), FHS in black ({\color{black}{ $\boldsymbol{-}$ }}), and benchmark buy and hold in grey ({\color{grey}{ $\boldsymbol{-}$ }}) color.}
\label{fig:exthree}
\end{sidewaysfigure}



\begin{figure}[!h]
\centering
\includegraphics[width=0.8\textwidth]{Relative_performance_figure}
\caption{Relative performance: trading strategy based on probability predictions from ordered logit model relative to separate logits (top right) as well as benchmark market (top left), GARCH (bottom left), and FHS (bottom right). Median value from all 29 stocks in black line surrounded with 90\% of distribution in grey area. Note that value of one shows equal performance of both strategies compared.}
\label{fig:relative}
\end{figure}


\clearpage
\newpage
\section{Figures: Sensitivity to Polynomial Orders}

\begin{figure}[!h]
\centering
\includegraphics[width=0.45 \textwidth]{BIC}
\caption{Bayesian information criterion for ordered logit model with different polynomial orders $(q_1\,q_2)$ on $x$-axis shown by box-and-whisker plots for all 29 stocks.}
\label{fig:sensitivityplot}
\end{figure}






